A candidate magnetic helium core white dwarf in the globular cluster NGC 6397

We report a peculiar variable blue star in the globular cluster NGC 6397, using Hubble Space Telescope optical imaging. Its position in the colour-magnitude diagrams, and its spectrum, are consistent with this star being a helium core white dwarf (He WD) in a binary system. The optical light curve shows a periodicity at 18.5 hours. We argue that this periodicity is due to the rotation of the WD and possibly due to magnetic spots on the surface of the WD. This would make this object the first candidate magnetic He WD in any globular cluster (GC), and the first candidate magnetic WD in a detached binary system in any GC and one of the few He WDs with a known rotation period and of magnetic nature. Another possibility is that this system is a He WD in a binary system with another WD or another degenerate object, which would make this object one of the few candidate non-accreting double degenerate binaries in any GC.

==> Notas.tex <==


\begin{comment}
    
    The observation by 
  \cite{cool_discovery_1993} first detected X-ray sources in NGC 6397, with the {\it ROSAT} satellite. %Since then 
  Optical and UV observations with the {\it Hubble Space Telescope} (HST) have enabled the identification of several X-ray sources with blue, variable, and/or H$\alpha$ bright stars \citep{cool_discovery_1995,grindlay_spectroscopic_1995,Cool98,taylor_helium_2001,Ferraro01,Shara05}. Identifications were dramatically improved by the  sub-arcsecond positions of the {\it Chandra X-ray Observatory} \citep{grindlay_chandra_2001,bogdanov_chandra_2010}, enabling identification of many more optical/UV counterparts with HST \citep{kaluzny_photometric_2006,cohn_identification_2010,Heinke14,Pallanca2017Halpha,Dieball2017UV}.
  %Follow-up observations with {\it Chandra} \citep{grindlay_chandra_2001,bogdanov_chandra_2010} and {\it Hubble} \citep{taylor_helium_2001,2006Sci...313..936R,grindlay_compact_2006} have identified their probable optical counterparts, and determined whether they show H$\alpha$ emission \citep{cohn_identification_2010,Pallanca2017Halpha}.
%Mention here the know redbacks in cluster. 
NGC~6397 has also been observed with radio telescopes, both imaging observations with the {\it Australia Telescope Compact Array} ({\it ATCA}) \citep{CoryPaper}, and %timing observation 
radio pulsar searches 
with Parkes \citep{damico2001discovery} that 
%confirmed the nature of 
discovered PSR J1740-5340  (aka the X-ray source U12, \citealt{grindlay_chandra_2001}) and confirmed its nature as an eclipsing redback system. 


\cite{Caiazzo2020ApJ...901L..14C} reported "the discovery of two massive and magnetic white-dwarf members of young star clusters in the Gaia second data release (DR2) database, while a third massive and magnetic cluster white dwarf was already reported in a previous paper."


first one found by \cite{Richer2021ApJ...912..165R} but


from literature searched 

 "A search in the literature reveals the existence of four more binary systems that include a magnetic white dwarf
and a non-degenerate companion; three such systems passed unremarked in previous studie" from \cite{Landstreet2020A&A...634L..10L} and "Thus it is clear that although only a few binary systems
including an MWD and a non-degenerate star have been iden-
tified, several are found even within the solar neighbourhood."

%They "All three WDs have quite high masses (around 1 M) and progenitor masses of around 5 or 6 M. Caiazzo et al. (2020) argue that these new MWDs are so young that it is very unlikely that they formed from binary merger
%processes discussed in Section 7.2.3; instead they are almost certainly
%descended from single upper MS stars. These discoveries, if fully
%confirmed, appear to require that at least some MWDs descend from
%single MS stars."





Theoretical work by \cite{Schreiber2021NatAs...5..648S} and also

by \cite{Kremer2021ApJ...917...28K}



Serach for He core WDs in NGC~6397 by \cite{Strickler2009ApJ...699...40S}


Long period roation of 1. 4 days \cite{Brinkworth2005MNRAS.357..333B}




About pulsation: "We detected a significant pulsation mode in GD 278
at 6729.0 ± 1.8 s, which is so far the longest pul-
sation period detected in a white dwarf. Previously,
SDSS J222859.93+362359.6 had the longest detected pul-
sation period at 6234.9 ± 6.0 s" in \cite{Lopez2021ApJ...922..220L}


Interested: " Magnetic white dwarfs in post-common-envelope binaries " in \cite{Parsons2021MNRAS.502.4305P}


progenitors not much magnetism : \cite{Liebert2005AJ....129.2376L} and \cite{Liebert2015ApJ...804...93L}



%$30 \%  $ is binary "However, < ∼ 20−30 per cent of the low-mass
%WDs seem to be single (Brown et al., 2011),\cite{Brown ApJ...730...67B}



%Extremely low-mass white dwarfs (ELM WDs) are here defined as helium-core WDs with masses M ≲ 0.18 M⊙, sufficiently low that no hydrogen shell flashes occur during the WD cooling stage. 

%First pulsator and quite high applitude \cite{Hermes2012ApJ...750L..28H}


%Pulsating amplitude "0.010.3 mag." ZZ Ceti


%99 minutes to 17.9 days \cite{SchmidtWDMagnetic1991ApJ...366..270S,RotationMagWDBrinkworth2013ApJ...773...47B}.

% 11228 % CMDID0011228
%HackID10097.0

\end{comment}


%Althoug they can be fomre from single 
%Castellani
%He WDs are thought to be product of binary evolution and part of the compact binary population in GCs. He WDs can also be formed from single stars if they can somehow lose an unusually large amount of mass while on the RGB (Castellani & Castellani 1993). However, as we will show, the radial distribution of the He WDs in NGC 6397 strongly suggests that they have binary companions, making such scenarios unlikely to apply in this case.



%Double-degenerate He WD binaries are of additional interest as potential progenitors of AM CVn stars (Nelemans et al. 2001a)and sources of gravitational radiation (Benacquista 2006, refer to Section 6).


%Characterizing the population of He core WDs is important 





%He WDs in NGC~6397 were first identified by \cite{Cool98} as nonflickering UV stars. These stars were later identify via spectroscopy \cite{edmonds_cataclysmic_1999} as good candidate low-mass He WDs. More recently  \cite{taylor_helium_2001} and \cite{Strickler2009ApJ...699...40S} expanded the list of possible He WDs candidates in NGC~6397 

%Taylor et al. 2001). The spectrum of NF2,with its apparently Doppler-shifted Hβ line, also hints at the influence of a dark, compact companion (Edmonds et al. 1999). Double-degenerate He WD binaries are of additional interest as potential progenitors of AM CVn stars (Nelemans et al. 2001a)and sources of gravitational radiation (Benacquista 2006, refer to Section 6).


\begin{comment}
    
    

    

Yet another marker of compact binary populations in globulars are helium white dwarfs (He WDs). As the stripped cores of (sub)giants, He WDs are a natural outcome of compact binary evolution. Three objects in NGC 6397 were first identified by Cool et al. (1998, hereafter CGC) as stars significantly bluer than the main sequence (MS) but lacking the flicker variations generally seen in CVs. Follow-up HST/Faint Object Spectrograph observations by Edmonds et al. (1999, hereafter EGC) of one of these "nonflickerers" (NF 2) yielded a spectrum consistent with an He WD and 247 ± 50 km s-1 Doppler shift—suggesting it is in a binary with a dark companion, most probably a massive WD or an NS and by implication that the other NFs might also be He WDs. While He WDs have been observed directly as the optical counterparts and secondaries of binary MSPs in the field (e.g., van Kerkwijk, Bergeron, & Kulkarni 1996), this was the first to be found in a globular cluster.


\end{comment}


%\cite{Strickler2009ApJ...699...40S} estimated a mass range for the 24 He WD candidates to be between $\sim 0.2-0.3  M_\odot$. This agrees with the estimated mass for the spectroscopically confirmed He WD with a mass of $0.25 M_\odot$ \cite{edmonds_cataclysmic_1999}. Given this mass range, a radial velocity of $\sim 250$ km/s, and an orbital period of 0.76 days would give a lower limit for the companion mass of $\sim 1.23 M_\odot$. 


%the upper limit from the brightness is fainter than the lower limit from the mass function



% close to 30". 
%Outside the core radius:
%0.05 arcmin from Harris is the core radius
%distance from the center is about 17. times the core radius
%51.38820673314435 arcsecond from the center or about 17.12940224438145 

